Determination of the Number of Topics Intrinsically: Is It Possible?

The number of topics might be the most important parameter of a topic model. The topic modelling community has developed a set of various procedures to estimate the number of topics in a dataset, but there has not yet been a sufficiently complete comparison of existing practices. This study attempts to partially fill this gap by investigating the performance of various methods applied to several topic models on a number of publicly available corpora. Further analysis demonstrates that intrinsic methods are far from being reliable and accurate tools. The number of topics is shown to be a method- and a model-dependent quantity, as opposed to being an absolute property of a particular corpus. We conclude that other methods for dealing with this problem should be developed and suggest some promising directions for further research.

==> pieces.tex <==

All experiments were conducted in order to find out whether it is possible to determine the number of topics in a dataset.
The number of topics is a topic model hyperparameter that must be set before model training.
Thus, determining the number of topics is a separate problem.



From the graphs of the dependence of the model scores on the number of topics
\ref{}  % TODO
it can be seen that there is no such intrinsic model quality criterion by which it would be possible to determine the number of topics.
An indicator of the optimum could be a local minimum (or local maximum~---~depending on the score), but in most cases the dependencies are either monotonous or jumping.
One can also notice that different topic models have different dependencies of scores on the number of topics, and the difference is not only in amplitude
\ref{}.  % TODO
The success in determining the optimal number of topics also depends on the dataset.
For example, the
SOME MODEL  % TODO
managed to find the optimum in number of topics for the
SOME DATASET but for the OTHER DATASET  % TODO x2
it did not \ref{}. % TODO

Similarly with stability experiments.
Different models may give different results.
And, although the stability estimates did show some numbers of topics which gave local optimum in stability, the expected number of topics was usually far lower than points which gave local optimum (maybe due to disbalance in the natural language text collections that were used).  % TODO: check info, look at plots
For some datasets, there are distinct optimums (when a descent is observed for at least several points on the left and rise~---~on the right).

Determining the number of topics using renormalization turned out to be highly dependent on the hyperparameter $\mathrm{threshold}$, which is taken literally from nowhere.
By setting different thresholds, one can obtain as a result significantly different numbers of topics for the same dataset and topic model; bigger thresholds generally lead to higher optimal number of topics found by the search method
\ref{}.  % TODO


The ways to evaluate this optimal number of topics using intrinsic model quality criteria do not inspire confidence.


Thus, conducted experiments show that the optimal number of topics depends not only on the dataset itself but also on the topic model being used.
If speaking about extrinsic topic model quality criteria, then, obviously, the optimal number of topics will depend on which task is solved by topic modeling.
For example, one can get generally interpretable topic models with different numbers of topics, but for the external task at hand some topic models will be more useful than others \cite{ianina2017multi}.

It is worth emphasizing that the notion of optimal number of topics is highly dependent on the dataset topic structure, on the disbalance of topics \cite{veselova2020topic}.
Thus, if it was possible to obtain an estimate of the optimal number of topics, then it was close to the expected value in the case of balanced datasets and less than the expected value in the case of unbalanced datasets.



% \footnote{We take $10$ most frequent tags as the first approximation to the set of topics. Next we add most frequent remaining tag unless it significantly overlaps with the existing topics. Depending on precise thresholds, one can obtain 15 to 28 clusters with this process.}. 


% Topic modeling helps to find hidden topics in a collection of text documents.
% However, the number of topics is a hyperparameter of topic models, which, proceeding from some considerations, needs to be fixed before model training.
% In research works, some ways were suggested to estimate the number of topics in a dataset: by observing some characteristics of a topic model depending on the number of topics.
% However, there has not yet been a sufficiently complete comparison of existing practices to determine the number of topics.
% The presented work is just dedicated to filling this gap.
% We selected several publicly available sets of natural language texts and fixed a range of topic models for further training.
% Then, we implemented several ways to determine the number of topics in a dataset and applied them to find the number of topics when training a specific model on a specific dataset.


